Accurate and numerically efficient r$^2$SCAN meta-generalized gradient approximation

The recently proposed rSCAN functional [J. Chem. Phys. 150, 161101 (2019)] is a regularized form of the SCAN functional [Phys. Rev. Lett. 115, 036402 (2015)] that improves SCAN's numerical performance at the expense of breaking constraints known from the exact exchange-correlation functional. We construct a new meta-generalized gradient approximation by restoring exact constraint adherence to rSCAN. The resulting functional maintains rSCAN's numerical performance while restoring the transferable accuracy of SCAN.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> norms_table.tex <==
    \begin{tabular}{cl|rrrrrr}
    \hline
    \hline
                           &                & \multicolumn{1}{c}{SCAN} & \multicolumn{1}{c}{rSCAN} & \multicolumn{1}{c}{r++SCAN} & \multicolumn{1}{c}{r$^2$SCAN} & \multicolumn{1}{c}{r$^4$SCAN} \\
\hline
\multirow{3}{*}{\shortstack{Rare\\Gas}} & $E_{\mr{x}}$ &     0.29\% &     0.44\% &     0.40\% &     0.12\% &     0.13\% \\
 & $E_{\mr{c}}$ &     6.29\% &     5.86\% &     5.71\% &     5.37\% &     5.37\% \\
 & $E_{\mr{xc}}$ &     0.13\% &     0.28\% &     0.24\% &     0.10\% &     0.02\% \\
\hline
\multirow{3}{*}{\shortstack{Jellium\\Surface}} & $E_{\mr{x}}$ &    24.50\% &  2239.33\% &    46.79\% &    40.80\% &    38.49\% \\
 & $E_{\mr{c}}$ &    35.03\% &  1499.79\% &    51.32\% &    49.48\% &    49.48\% \\
 & $E_{\mr{xc}}$ &     5.02\% &   228.45\% &     3.46\% &     3.12\% &     2.35\% \\
\hline
\multicolumn{2}{c|}{Ar\mol{2}}  &     1.07\% &     0.71\% &     0.90\% &     0.62\% &     0.81\% & \\
\hline
\hline
\end{tabular}
